Real-time Video Summarization on Commodity Hardware

We present a method for creating video summaries in real-time on commodity hardware. Real-time here refers to the fact that the time required for video summarization is less than the duration of the input video. First, low-level features are use to discard undesirable frames. Next, video is divided into segments, and segment-level features are extracted for each segment. Tree-based models trained on widely available video summarization and computational aesthetics datasets are then used to rank individual segments, and top-ranked segments are selected to generate the final video summary. We evaluate the proposed method on SUMME dataset and show that our method is able to achieve summarization accuracy that is comparable to that of a current state-of-the-art deep learning method, while posting significantly faster run-times. Our method on average is able to generate a video summary in time that is shorter than the duration of the video.

==> figures/sampling-all-leave-one-out.tex <==
\begin{tikzpicture}[scale=0.95]
\coordinate (base) at (0, 0);
\DrawVideo{blue!50!white}{0.00386672180456}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00249298700136}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00206884932627}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213836077858}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0021147975744}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00737057026489}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0037477276235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00419307218234}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228798712507}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213600445816}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00296307292458}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00315393487837}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00383962411977}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00495416367709}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00275218224725}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00497301424042}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00401870447147}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00537947951238}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00618180661443}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00346379101323}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00325290033589}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00314686591712}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0056422092389}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286175114664}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286057298644}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00423077330902}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00254600421074}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00435565829113}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00425315835298}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00568108852578}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00345083125094}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0042566928336}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00221376303192}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00339781404155}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00204999876293}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00273686616453}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00405876191856}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00374419314287}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00247884907886}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00246117667573}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00266617655202}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00307971078523}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00271565928078}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00624307094527}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00322109001026}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00256367661387}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00319281416526}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228445264444}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00424962387235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00165531509306}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00529465197737}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00557151962638}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00393623325687}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00360988287909}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00604514003023}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00597916305855}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0106576372468}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00151511402824}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00585663439686}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0114528953876}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00189919425623}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00111925219815}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00375479658475}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00542896224114}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00718206463151}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0036110610393}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00787364467395}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00261669382326}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00206295852523}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00455123288575}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0113951655374}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00610051356003}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.005162698034}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00303258437689}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00367585985077}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00814344336172}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00416126185671}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00676499591767}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00571761149225}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00471853163537}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00390206661082}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00552321505783}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0124849637303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0159181225781}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0180340983128}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00346496917344}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00699709347877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00513206586858}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0113939873772}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00688752457937}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0165166279641}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00447936511303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00507080153773}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00735289786176}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00558447938868}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00775229417247}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0128619749971}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00490821542895}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00637620304884}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0112337575888}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0093769771001}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00663422013452}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00391973901395}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0114646769897}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0052581290109}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00470675003328}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00666956494078}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00436508357279}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0228633770077}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00580950798852}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0206496139758}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00849453510387}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00553735298033}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00294540052145}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00703479460544}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00459011217263}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0134475206207}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00951128736388}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00526401981194}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0047232442762}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0116284412587}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0157461111877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00825890306216}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00509436474191}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00975634468726}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00256838925471}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0027180156012}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0062878410332}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00692169122542}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00978815501289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00992246527667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00505430729481}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00732462201675}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00142086121155}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00106505682856}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0124107396372}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00969390219621}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0157296169448}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00704186356669}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0102829823005}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0268314205902}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00258723981804}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00491057174937}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0108638152833}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0016612058941}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00553853114054}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00674614535434}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0187421725981}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0018944816154}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00305850390148}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00185795864893}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0184747302308}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00438157781571}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00492235335145}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0033907450803}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00632672032008}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0035827851943}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00384787124123}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00086359143289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.011675567667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00529229565695}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00033224117882}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0151864850886}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00482456605414}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00381134827476}{DatasetColorYoutube}
\coordinate (base) at (0, 0);
\DrawDataset{0.175648371017}
\DrawDataset{0.129385554106}
\DrawDataset{0.415130640295}
\DrawDataset{0.279835434582}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/sampling-leave-one-segment-out.tex <==
\begin{tikzpicture}[scale=0.95]
\coordinate (base) at (0, 0);
\DrawVideo{blue!50!white}{0.00386672180456}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00249298700136}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00206884932627}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213836077858}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0021147975744}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00737057026489}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0037477276235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00419307218234}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228798712507}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213600445816}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00296307292458}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00315393487837}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00383962411977}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00495416367709}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00275218224725}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00497301424042}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00401870447147}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00537947951238}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00618180661443}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00346379101323}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00325290033589}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00314686591712}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0056422092389}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286175114664}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286057298644}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00423077330902}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00254600421074}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00435565829113}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00425315835298}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00568108852578}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00345083125094}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0042566928336}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00221376303192}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00339781404155}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00204999876293}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00273686616453}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00405876191856}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00374419314287}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00247884907886}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00246117667573}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00266617655202}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00307971078523}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00271565928078}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00624307094527}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00322109001026}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00256367661387}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00319281416526}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228445264444}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00424962387235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00165531509306}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00529465197737}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00557151962638}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00393623325687}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00360988287909}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00604514003023}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00597916305855}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0106576372468}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00151511402824}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00585663439686}{DatasetColorSUMME}
% Three segments
\DrawVideo{blue!50!white}{0.0034528953876}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0054528953876}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0034528953876}{DatasetColorSUMME}
%
\DrawVideo{blue!50!white}{0.00189919425623}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00111925219815}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00375479658475}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00542896224114}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00718206463151}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0036110610393}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00787364467395}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00261669382326}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00206295852523}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00455123288575}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0113951655374}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00610051356003}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.005162698034}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00303258437689}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00367585985077}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00814344336172}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00416126185671}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00676499591767}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00571761149225}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00471853163537}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00390206661082}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00552321505783}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0124849637303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0159181225781}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0180340983128}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00346496917344}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00699709347877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00513206586858}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0113939873772}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00688752457937}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0165166279641}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00447936511303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00507080153773}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00735289786176}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00558447938868}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00775229417247}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0128619749971}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00490821542895}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00637620304884}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0112337575888}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0093769771001}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00663422013452}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00391973901395}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0114646769897}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0052581290109}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00470675003328}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00666956494078}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00436508357279}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0228633770077}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00580950798852}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0206496139758}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00849453510387}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00553735298033}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00294540052145}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00703479460544}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00459011217263}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0134475206207}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00951128736388}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00526401981194}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0047232442762}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0116284412587}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0157461111877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00825890306216}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00509436474191}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00975634468726}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00256838925471}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0027180156012}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0062878410332}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00692169122542}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00978815501289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00992246527667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00505430729481}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00732462201675}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00142086121155}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00106505682856}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0124107396372}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00969390219621}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0157296169448}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00704186356669}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0102829823005}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0268314205902}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00258723981804}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00491057174937}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0108638152833}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0016612058941}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00553853114054}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00674614535434}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0187421725981}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0018944816154}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00305850390148}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00185795864893}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0184747302308}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00438157781571}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00492235335145}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0033907450803}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00632672032008}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0035827851943}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00384787124123}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00086359143289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.011675567667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00529229565695}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00033224117882}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0151864850886}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00482456605414}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00381134827476}{DatasetColorYoutube}
\coordinate (base) at (0, 0);
\DrawDataset{0.175648371017}
\DrawDataset{0.129385554106}
\DrawDataset{0.415130640295}
\DrawDataset{0.279835434582}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/sampling-other-datasets.tex <==
\begin{tikzpicture}[scale=0.95]
\coordinate (base) at (0, 0);
\DrawVideo{blue!50!white}{0.00386672180456}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00249298700136}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00206884932627}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213836077858}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0021147975744}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00737057026489}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0037477276235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00419307218234}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228798712507}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00213600445816}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00296307292458}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00315393487837}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00383962411977}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00495416367709}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00275218224725}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00497301424042}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00401870447147}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00537947951238}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00618180661443}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00346379101323}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00325290033589}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00314686591712}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0056422092389}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286175114664}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00286057298644}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00423077330902}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00254600421074}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00435565829113}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00425315835298}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00568108852578}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00345083125094}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.0042566928336}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00221376303192}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00339781404155}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00204999876293}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00273686616453}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00405876191856}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00374419314287}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00247884907886}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00246117667573}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00266617655202}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00307971078523}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00271565928078}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00624307094527}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00322109001026}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00256367661387}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00319281416526}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00228445264444}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00424962387235}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00165531509306}{DatasetColorOpenvideo}
\DrawVideo{red!50!white}{0.00529465197737}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00557151962638}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00393623325687}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00360988287909}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00604514003023}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00597916305855}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0106576372468}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00151511402824}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00585663439686}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0114528953876}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00189919425623}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00111925219815}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00375479658475}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00542896224114}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00718206463151}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0036110610393}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00787364467395}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00261669382326}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00206295852523}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00455123288575}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0113951655374}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00610051356003}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.005162698034}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00303258437689}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.00367585985077}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00814344336172}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00416126185671}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00676499591767}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00571761149225}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00471853163537}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00390206661082}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00552321505783}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0124849637303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0159181225781}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0180340983128}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00346496917344}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00699709347877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00513206586858}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0113939873772}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00688752457937}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0165166279641}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00447936511303}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00507080153773}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00735289786176}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00558447938868}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00775229417247}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0128619749971}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00490821542895}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00637620304884}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0112337575888}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0093769771001}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00663422013452}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00391973901395}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0114646769897}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0052581290109}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00470675003328}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00666956494078}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00436508357279}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0228633770077}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00580950798852}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0206496139758}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00849453510387}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00553735298033}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00294540052145}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00703479460544}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00459011217263}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0134475206207}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00951128736388}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00526401981194}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0047232442762}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0116284412587}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.0157461111877}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00825890306216}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00509436474191}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00975634468726}{DatasetColorTVSUM50}
\DrawVideo{blue!50!white}{0.00256838925471}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0027180156012}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0062878410332}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00692169122542}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00978815501289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00992246527667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00505430729481}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00732462201675}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00142086121155}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00106505682856}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0124107396372}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00969390219621}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0157296169448}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00704186356669}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0102829823005}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0268314205902}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00258723981804}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00491057174937}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0108638152833}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0016612058941}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00553853114054}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00674614535434}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0187421725981}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0018944816154}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00305850390148}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00185795864893}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0184747302308}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00438157781571}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00492235335145}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0033907450803}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00632672032008}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0035827851943}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00384787124123}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00086359143289}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.011675567667}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00529229565695}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00033224117882}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.0151864850886}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00482456605414}{DatasetColorYoutube}
\DrawVideo{blue!50!white}{0.00381134827476}{DatasetColorYoutube}
\coordinate (base) at (0, 0);
\DrawDataset{0.175648371017}
\DrawDataset{0.129385554106}
\DrawDataset{0.415130640295}
\DrawDataset{0.279835434582}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> figures/sampling-same-leave-one-out.tex <==
\begin{tikzpicture}[scale=0.95]
\coordinate (base) at (0, 0);
\DrawVideo{white}{0.00386672180456}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00249298700136}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00206884932627}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00213836077858}{DatasetColorOpenvideo}
\DrawVideo{white}{0.0021147975744}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00737057026489}{DatasetColorOpenvideo}
\DrawVideo{white}{0.0037477276235}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00419307218234}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00228798712507}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00213600445816}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00296307292458}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00315393487837}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00383962411977}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00495416367709}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00275218224725}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00497301424042}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00401870447147}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00537947951238}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00618180661443}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00346379101323}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00325290033589}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00314686591712}{DatasetColorOpenvideo}
\DrawVideo{white}{0.0056422092389}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00286175114664}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00286057298644}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00423077330902}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00254600421074}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00435565829113}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00425315835298}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00568108852578}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00345083125094}{DatasetColorOpenvideo}
\DrawVideo{white}{0.0042566928336}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00221376303192}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00339781404155}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00204999876293}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00273686616453}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00405876191856}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00374419314287}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00247884907886}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00246117667573}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00266617655202}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00307971078523}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00271565928078}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00624307094527}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00322109001026}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00256367661387}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00319281416526}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00228445264444}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00424962387235}{DatasetColorOpenvideo}
\DrawVideo{white}{0.00165531509306}{DatasetColorOpenvideo}
\DrawVideo{blue!50!white}{0.00529465197737}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00557151962638}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00393623325687}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00360988287909}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00604514003023}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00597916305855}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0106576372468}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00151511402824}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00585663439686}{DatasetColorSUMME}
\DrawVideo{red!50!white}{0.0114528953876}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00189919425623}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00111925219815}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00375479658475}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00542896224114}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00718206463151}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0036110610393}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00787364467395}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00261669382326}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00206295852523}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00455123288575}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.0113951655374}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00610051356003}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.005162698034}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00303258437689}{DatasetColorSUMME}
\DrawVideo{blue!50!white}{0.00367585985077}{DatasetColorSUMME}
\DrawVideo{white}{0.00814344336172}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00416126185671}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00676499591767}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00571761149225}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00471853163537}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00390206661082}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00552321505783}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0124849637303}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0159181225781}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0180340983128}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00346496917344}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00699709347877}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00513206586858}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0113939873772}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00688752457937}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0165166279641}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00447936511303}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00507080153773}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00735289786176}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00558447938868}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00775229417247}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0128619749971}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00490821542895}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00637620304884}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0112337575888}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0093769771001}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00663422013452}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00391973901395}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0114646769897}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0052581290109}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00470675003328}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00666956494078}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00436508357279}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0228633770077}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00580950798852}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0206496139758}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00849453510387}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00553735298033}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00294540052145}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00703479460544}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00459011217263}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0134475206207}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00951128736388}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00526401981194}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0047232442762}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0116284412587}{DatasetColorTVSUM50}
\DrawVideo{white}{0.0157461111877}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00825890306216}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00509436474191}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00975634468726}{DatasetColorTVSUM50}
\DrawVideo{white}{0.00256838925471}{DatasetColorYoutube}
\DrawVideo{white}{0.0027180156012}{DatasetColorYoutube}
\DrawVideo{white}{0.0062878410332}{DatasetColorYoutube}
\DrawVideo{white}{0.00692169122542}{DatasetColorYoutube}
\DrawVideo{white}{0.00978815501289}{DatasetColorYoutube}
\DrawVideo{white}{0.00992246527667}{DatasetColorYoutube}
\DrawVideo{white}{0.00505430729481}{DatasetColorYoutube}
\DrawVideo{white}{0.00732462201675}{DatasetColorYoutube}
\DrawVideo{white}{0.00142086121155}{DatasetColorYoutube}
\DrawVideo{white}{0.00106505682856}{DatasetColorYoutube}
\DrawVideo{white}{0.0124107396372}{DatasetColorYoutube}
\DrawVideo{white}{0.00969390219621}{DatasetColorYoutube}
\DrawVideo{white}{0.0157296169448}{DatasetColorYoutube}
\DrawVideo{white}{0.00704186356669}{DatasetColorYoutube}
\DrawVideo{white}{0.0102829823005}{DatasetColorYoutube}
\DrawVideo{white}{0.0268314205902}{DatasetColorYoutube}
\DrawVideo{white}{0.00258723981804}{DatasetColorYoutube}
\DrawVideo{white}{0.00491057174937}{DatasetColorYoutube}
\DrawVideo{white}{0.0108638152833}{DatasetColorYoutube}
\DrawVideo{white}{0.0016612058941}{DatasetColorYoutube}
\DrawVideo{white}{0.00553853114054}{DatasetColorYoutube}
\DrawVideo{white}{0.00674614535434}{DatasetColorYoutube}
\DrawVideo{white}{0.0187421725981}{DatasetColorYoutube}
\DrawVideo{white}{0.0018944816154}{DatasetColorYoutube}
\DrawVideo{white}{0.00305850390148}{DatasetColorYoutube}
\DrawVideo{white}{0.00185795864893}{DatasetColorYoutube}
\DrawVideo{white}{0.0184747302308}{DatasetColorYoutube}
\DrawVideo{white}{0.00438157781571}{DatasetColorYoutube}
\DrawVideo{white}{0.00492235335145}{DatasetColorYoutube}
\DrawVideo{white}{0.0033907450803}{DatasetColorYoutube}
\DrawVideo{white}{0.00632672032008}{DatasetColorYoutube}
\DrawVideo{white}{0.0035827851943}{DatasetColorYoutube}
\DrawVideo{white}{0.00384787124123}{DatasetColorYoutube}
\DrawVideo{white}{0.00086359143289}{DatasetColorYoutube}
\DrawVideo{white}{0.011675567667}{DatasetColorYoutube}
\DrawVideo{white}{0.00529229565695}{DatasetColorYoutube}
\DrawVideo{white}{0.00033224117882}{DatasetColorYoutube}
\DrawVideo{white}{0.0151864850886}{DatasetColorYoutube}
\DrawVideo{white}{0.00482456605414}{DatasetColorYoutube}
\DrawVideo{white}{0.00381134827476}{DatasetColorYoutube}
\coordinate (base) at (0, 0);
\DrawDataset{0.175648371017}
\DrawDataset{0.129385554106}
\DrawDataset{0.415130640295}
\DrawDataset{0.279835434582}
\end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

